MISO: Multiresolution Submap Optimization for Efficient Globally Consistent Neural Implicit Reconstruction

Neural implicit representations have had a significant impact on simultaneous localization and mapping (SLAM) by enabling robots to build continuous, differentiable, and high-fidelity 3D maps from sensor data. However, as the scale and complexity of the environment increase, neural SLAM approaches face renewed challenges in the back-end optimization process to keep up with runtime requirements and maintain global consistency. We introduce MISO, a hierarchical optimization approach that leverages multiresolution submaps to achieve efficient and scalable neural implicit reconstruction. For local SLAM within each submap, we develop a hierarchical optimization scheme with learned initialization that substantially reduces the time needed to optimize the implicit submap features. To correct estimation drift globally, we develop a hierarchical method to align and fuse the multiresolution submaps, leading to substantial acceleration by avoiding the need to decode the full scene geometry. MISO significantly improves computational efficiency and estimation accuracy of neural signed distance function (SDF) SLAM on large-scale real-world benchmarks.

==> sections/memory_measure.tex <==

\input{tables/memory_measure}

==> sections/notes.tex <==
%!TEX root = ../main.tex
\section{Earlier Ideas}

Our goal is to design transformations $\Tcal$ between grid models of different resolutions, so that
\begin{equation}
G^{l+1} = \Tcal_{l}^{l+1} \left[ G^l \right],
\end{equation}
at a given layer $l$.

\subsection{Wavelet}

Related to recent approaches \cite{rho2023masked,khatib2024trinerflet},
we consider the representation of the feature grids $F$ using its wavelet coefficients:
\begin{equation}
W = \dwt(F),
\end{equation}
where $\dwt$ is the Discrete Wavelet Transform.
We leverage the fact that both $\dwt$ and its inverse transform $\idwt$ are differentiable.
Therefore, we can optimize $W$ instead of the original feature grids $F$.
For example, for \cref{prob:sdf}, we can solve
\begin{equation}
	\label{eq:prob_sdf_wavelet}
	\underset{W}{\min}
	\quad \sum_{(p, s_p) \in D} \norm{
	D_\theta \left[ \Interp(p; \blue{\idwt(W)} ) \right] - s_p
	}^2.
\end{equation}
The main motivation is that $W$ is naturally organized into groups representing a coarse approximation and multiple levels of details:
\begin{equation}
W = \{ W_c, W_{d_1}, \hdots, W_{d_L} \}.
\end{equation}
When optimizing \eqref{eq:prob_sdf_wavelet}, we can fix or regularize some of these groups to achieve compression or faster convergence.

\subsection{Multigrid} 

Recall $V$ is the set of vertices on the original (dense) grid.
We will introduce a hierarchy of vertices:
\begin{equation}
    V \equiv V_0 \supseteq V_1 \supseteq V_2 \hdots \supseteq V_L,
\end{equation}
where $V_{l+1}$ are the vertices of a coarser grid, sampled from $V_l$.
Furthermore, let $F_l$ denote the set of all features at level $l \in \Natural$.
Given current features $\Fhat$, we want to improve by finding a correction/residual term $\Delta_F$.
For example, for \cref{prob:sdf}, this is formulated as: 
\begin{equation}
	\underset{\Delta_F}{\min}
	\quad \sum_{(p, s_p) \in D} \norm{
	D_\theta \left[ \Interp(p; \blue{\Fhat + \Delta_F} ) \right] - s_p
	}^2.
\end{equation}
The essence of multigrid is to transform the above into a lower dimensional problem defined on one of the coarser grids. 
Specifically, suppose level $l$ is selected as the approximation level.
Each level comes with an interpolation matrix such that:
\begin{equation}
    \Delta_F \equiv \Delta_F^{(0)}  = P_l \Delta_F^{(l)},
\end{equation}
where $\Delta_F^{(l)}$ is a lower-dimensional correction term.
The compressed problem is then,
\begin{equation}
	\underset{\blue{\Delta_F^{(l)}}}{\min}
	\quad \sum_{(p, s_p) \in D} \norm{
	D_\theta \left[ \Interp(p; \blue{\Fhat + P_l \Delta_F^{(l)}} ) \right] - s_p
	}^2.
\end{equation}

\begin{remark}[Choosing coarse nodes at each level]
    To get started, we can follow the standard geometric multigrid recipe, which uniformly decreases the resolution by half.

    A more advanced version can select coarse nodes based on the feature values, \eg, we should keep more coarse nodes in regions 
    where the features changes drastically.
\end{remark}

\begin{remark}[Choosing interpolation $P_l$]
    The interpolation $P_l$ can be defined using existing methods (\eg, trilinear interpolation, kron reduction \cite{dorfler2012kron}) or \blue{can be learned}.  
    For the learning approach, a recent relevant work shows that the training dynamics of grid-based models evolve according to a linear ODE governed by a constant grid tangent kernel (GTK) matrix \cite{zhao2024grounding}.

    Inspired by \cite{chen2023neurbf}: does it make sense to determine $P_l$ separately for each channel of the feature vector? In \cite{chen2023neurbf}, this is done to encourage different channel to learn at different frequencies.
\end{remark}





\subsection{Reducing computation cost at coarse level}
Current formulations of wavelet and multigrid do not directly improve the computation cost at coarser levels.
This is because at coarser levels, we still need to evaluate the exact cost function.
\blue{As an initial idea to try, we can subsample a smaller training set from $D$ at coarse levels.}

==> tables/scannet_metric.tex <==
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.6}
\caption{Ablation study on hierarchical alignment on ScanNet \cite{dai2017scannet} 
from large initial errors of $10$~deg and $0.25$~m.
For each scene, we report the final submap rotation error (deg) and translation error (m) 
compared to ground truth. Results averaged over 10 trials. 
Best results are highlighted in \textbf{bold}.}
\label{tab:scannet_metric}
\begingroup
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|cc|cc|cc|}
\hline
\multicolumn{1}{|c|}{Scene} 
& \multicolumn{2}{c|}{0011} 
& \multicolumn{2}{c|}{0024} 
& \multicolumn{2}{c|}{0169} \\
\multicolumn{1}{|c|}{Method} 
& \multicolumn{1}{c}{Rot err$\downarrow$} & \multicolumn{1}{c|}{Tran err$\downarrow$}
& \multicolumn{1}{c}{Rot err$\downarrow$} & \multicolumn{1}{c|}{Tran err$\downarrow$}
& \multicolumn{1}{c}{Rot err$\downarrow$} & \multicolumn{1}{c|}{Tran err$\downarrow$} \\
\hline
\method{Cos sim.}
 & 7.13 & 0.14 & - & - & 3.87 & 0.1 \\
\method{L1 dist.}
 & 2.31 & 0.07 & - & - & 3.09 & 0.14 \\
\method{L2 dist.}
 & \textbf{2.25} & \textbf{0.06} & - & - & \textbf{1.14} & \textbf{0.04} \\
\hline
\end{tabular}%
}
\endgroup
\end{table}

